Late Central Engine Activity in GRB 180205A

We present optical photometry of the afterglow of the long GRB 180205A with the COATLI telescope from 217 seconds to about 5 days after the {\itshape Swift}/BAT trigger. We analyse this photometry in the conjunction with the X-ray light curve from {\itshape Swift}/XRT. The late-time light curves and spectra are consistent with the standard forward-shock scenario. However, the early-time optical and X-ray light curves show non-typical behavior; the optical light curve exhibits a flat plateau while the X-ray light curve shows a flare. We explore several scenarios and conclude that the most likely explanation for the early behavior is late activity of the central engine.

==> table2.tex <==
1 & 126.8284 & 11.5043 & 15.57 $\pm$ 0.00 & 15.04 $\pm$ 0.00 & 15.33 $\pm$ 1.38 \\
2 & 126.8023 & 11.5666 & 14.47 $\pm$ 0.00 & 13.90 $\pm$ 0.00 & 14.20 $\pm$ 1.39 \\
3 & 126.8176 & 11.5555 & 14.72 $\pm$ 0.00 & 14.36 $\pm$ 0.00 & 14.59 $\pm$ 1.39 \\
4 & 126.8128 & 11.5419 & 16.2 $\pm$ 0.00 & 15.76 $\pm$ 0.00 & 16.05 $\pm$ 1.39 \\
5 & 126.8352 & 11.5188 & 14.7 $\pm$ 0.00 & 14.47 $\pm$ 0.00 & 14.69 $\pm$ 1.38 \\
6 & 126.8128 & 11.5050 & 14.16 $\pm$ 0.00 & 13.57 $\pm$ 0.00 & 13.84 $\pm$ 1.38 \\
7 & 126.8230 & 11.4638 & 12.24 $\pm$ -999.00 & 12.04 $\pm$ -999.00 & 12.13 $\pm$ 1.38 \\

